Fact-Aware Multimodal Retrieval Augmentation for Accurate Medical Radiology Report Generation

Multimodal foundation models hold significant potential for automating radiology report generation, thereby assisting clinicians in diagnosing cardiac diseases. However, generated reports often suffer from serious factual inaccuracy. In this paper, we introduce a fact-aware multimodal retrieval-augmented pipeline in generating accurate radiology reports (FactMM-RAG). We first leverage RadGraph to mine factual report pairs, then integrate factual knowledge to train a universal multimodal retriever. Given a radiology image, our retriever can identify high-quality reference reports to augment multimodal foundation models, thus enhancing the factual completeness and correctness of report generation. Experiments on two benchmark datasets show that our multimodal retriever outperforms state-of-the-art retrievers on both language generation and radiology-specific metrics, up to 6.5% and 2% score in F1CheXbert and F1RadGraph. Further analysis indicates that employing our factually-informed training strategy imposes an effective supervision signal, without relying on explicit diagnostic label guidance, and successfully propagates fact-aware capabilities from the multimodal retriever to the multimodal foundation model in radiology report generation.

==> Sections/Acknowledge.tex <==
\section*{Acknowledgments}
\label{sec:Acknowledgments}

==> Tables/Ablation_chexpert.tex <==
\begin{table*}[t]

\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{4}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    \textbf{Backbone}  & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L   & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L  \\
    \midrule
    ClueWeb-LLaVA$_{1.5}$              & 0.467  & 0.491 & 0.174   & 0.237   & 0.473 & 0.495 & 0.180 & 0.239  \\
    WebQA-LLaVA$_{1.5}$           &  0.468 & 0.464  & 0.184   & 0.239  & 0.474 &0.456 &  0.184   &   0.237     \\
    Med-MARVEL-LLaVA$_{1.5}$      & 0.469& 0.482  & 0.177 & 0.234   &0.474    & 0.475   & 0.185  & 0.236   \\
    ClueWeb-LLaVA$_{1.6}$            & 0.467  & 0.491 & 0.174   & 0.237 & 0.471  & 0.492 & 0.178  & 0.237  \\
    \bottomrule
\end{tabular}
}
\caption{Backbone Ablation Results on CheXpert}
\label{tab:ablation_chexpert}
\end{table*}


==> Tables/Ablation_mimic.tex <==
% \begin{table*}[h]
% \caption{Backbone Ablation Results on MIMIC-CXR}
% \label{tab:ablation_mimic}
% \centering
% \resizebox{\textwidth}{!}{
% % jz: copied highlighted results here
% \begin{tabular}{lccccccccc}
%     \toprule
%     & \multicolumn{4}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{4}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     \textbf{Backbone}  & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L   & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L  \\
%     \midrule
%     ClueWeb-LLaVA$_{1.5}$              &  &  & 0.137   & 0.211  & 0.5436  & 0.4768 & 0.2328   & 0.2939  
%         \\
%     WebQA-LLaVA$_{1.5}$           & 0.489  & 0.341 & 0.16   & 0.238  & 0.5522  & 0.5071 & 0.2414   & 0.3006        \\
%     Med-MARVEL-LLaVA$_{1.5}$                 & 1.453  & 0.346 & 0.137   & 0.211  & 0.5436  & 0.4768 & 0.2328   & 0.2939  \\
%     ClueWeb-LLaVA$_{1.6}$             & 1.453  & 0.346 & 0.137   & 0.211  & 0.5436  & 0.4768 & 0.2328   & 0.2939  \\
%     \bottomrule
% \end{tabular}
% }
% \end{table*}
\begin{table*}[t]

\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{4}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    \textbf{Backbone}  & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L   & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L  \\
    \midrule
    ClueWeb-LLaVA$_{1.5}$               & 0.547  & 0.605 & 0.249   & 0.297  & 0.561 & 0.602 & 0.256 & 0.307   \\
    WebQA-LLaVA$_{1.5}$           & 0.554  & 0.574  & 0.257   & 0.300  & 0.562  & 0.572 & 0.262    & 0.304        \\
    Med-MARVEL-LLaVA$_{1.5}$                 &  0.551 & 0.581 & 0.253   &0.301   & 0.563  & 0.581 & 0.260    & 0.311   \\
    ClueWeb-LLaVA$_{1.6}$            & 0.547  & 0.605 & 0.249   & 0.297 & 0.558  & 0.601 & 0.252  & 0.303  \\
    \bottomrule
\end{tabular}
}
\caption{Backbone Ablation Results on MIMIC-CXR \cx{update this ablation following the main results}}
\label{tab:ablation_mimic}
\end{table*}


==> Tables/Chexpert.tex <==
\begin{table*}[h]

\centering
\resizebox{\textwidth}{!}{
% jz: copied highlighted results here
\begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{4}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    \textbf{Model} & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L  \\

    \midrule
    No Retriever & ----  & ---- & ----   & ----  & 0.469	& 0.371	& 0.173 & 0.231 \\
    \midrule
    GLoRIA    & 0.447 & 0.359 & 0.135   & 0.216 & 0.468  & 0.397 & 0.173   & 0.231  
        \\
    CLIP        & 0.439  & 0.285 & 0.130   & 0.207 & 0.468  & 0.381 & 0.172   & 0.231        \\
    BiomedCLIP         & 0.441 & 0.386 & 0.142   & 0.216  & 0.469  & 0.380 & 0.173   & 0.232       \\
    MedCLIP          & 0.454  & 0.478 & 0.161   & 0.225 & 0.471  & 0.408 & 0.182   & 0.238        \\
    CXR-CLIP            & 0.458  & 0.444 & 0.167   & 0.230 & 0.471  & 0.406 & 0.183   & 0.241 \\
    \midrule
    Med-MARVEL  & 0.454  & 0.479 & 0.160   & 0.222  & 0.472 & 0.454 & \textbf{0.185} & \textbf{0.243} \\
    FactMM-RAG  & \textbf{0.467 } & \textbf{0.491} & \textbf{0.174}   & \textbf{0.237}   & \textbf{0.473}&\textbf{0.495}&0.180&0.239\\
    \bottomrule
\end{tabular}
}
\caption{Overall performance of FactMM-RAG and baselines on CheXpert \cx{need variances in the table, or stat.sig. tests.}}
\label{tab:chexpert_major}
\end{table*}

==> Tables/Dataset_Stats.tex <==
\begin{table}
\centering
\small
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{lr}
    \toprule
    \textbf{Split} & \textbf{Size}\\\hline
    MIMIC-CXR Train & 125,417 \\
    MIMIC-CXR Validation & 991 \\
    MIMIC-CXR Test & 1,624 \\
    CheXpert Test & 1,000 \\
    \bottomrule
\end{tabular}
}
\caption{Dataset Statistics.}
\label{tab:dataset}
\end{table}

==> Tables/MIMIC-CXR-main.tex <==
\begin{table*}[h]

\centering
\resizebox{\textwidth}{!}{
% jz: copied highlighted results here
\begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{4}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    \textbf{Model} & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L & BERTScore & F1CheXbert & F1RadGraph & ROUGE-L \\
    \midrule
    No Retriever & ----  & ---- & ----   & ----  & 0.549	& 0.496	& 0.234 & 0.294 \\
    \midrule
    GLoRIA                & 0.453  & 0.346 & 0.137   & 0.211  & 0.543  & 0.476 & 0.232   & 0.294  \\
    CLIP          & 0.489  & 0.341 & 0.160   & 0.238  & 0.552  & 0.507 & 0.241   & 0.300        \\
    BiomedCLIP          & 0.498  & 0.413 & 0.180   & 0.250  & 0.546  & 0.502 & 0.233   & 0.293        \\
    MedCLIP            & 0.508  & 0.539 & 0.198   & 0.261  & 0.549  & 0.517 & 0.238   & 0.298         \\
    CXR-CLIP               & 0.524  & 0.516 & 0.215   & 0.277  & 0.553  & 0.501 & 0.243   & 0.302 \\
    \midrule
    Med-MARVEL  & 0.525  & 0.550 & 0.212   & 0.279  &  0.549&0.537&0.237 & 0.306\\

    FactMM-RAG  & \textbf{0.547}  & \textbf{0.605 }&\textbf{ 0.249}   & \textbf{0.297}  & \textbf{0.561} & \textbf{0.602} & \textbf{0.257} & \textbf{0.307} \\
    \bottomrule
\end{tabular}
}
\caption{Overall performance of FactMM-RAG and baselines on MIMIC-CXR \cx{We should focus on the RAG results, and move the retrieval 1-nn results only to ablation and analysis, we also don't need to show all 1-nn results.} \cx{merge the RAG results of two datasets into one table.} \cx{put BERTScore together with ROUGE-L and mark them as text similarity, and mark F1CheXbert and F1RadGraph to something as factual similarity} \cx{shall we add references to baselines?}}
\label{tab:mimic_major}
\end{table*}

==> Tables/Propagation.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
    \toprule
    & & \multicolumn{2}{c}{\textbf{Multimodal Retrieval}} & \multicolumn{2}{c}{\textbf{Multimodal Retrieval Augmented Generation}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    \textbf{Model}  &MRR$@100$& F1CheXbert & F1RadGraph & F1CheXbert & F1RadGraph  \\
    \midrule
    epoch 1         & 0.043   & 0.549 & 0.211 &  0.547& 0.229     \\
    epoch 2          & 0.055  & 0.530 & 0.230  &  0.518&0.245        \\
    epoch 3          & 0.070  & 0.578  & 0.237&  0.575&0.247   \\
    epoch 4           & 0.069 & 0.580& 0.234   &  0.578&0.245     \\
    epoch 5           & 0.076  &0.591  & 0.238  & 0.589  & 0.249    \\
    \bottomrule
\end{tabular}
}
\caption{Fact-aware Propagation from Retriever to Foundation Model \ls{pending to draw a figure for this}}
\label{tab:prop}
\end{table*}

